Learning Sparse Latent Representations with the Deep Copula Information Bottleneck

Deep latent variable models are powerful tools for representation learning. In this paper, we adopt the deep information bottleneck model, identify its shortcomings and propose a model that circumvents them. To this end, we apply a copula transformation which, by restoring the invariance properties of the information bottleneck method, leads to disentanglement of the features in the latent space. Building on that, we show how this transformation translates to sparsity of the latent space in the new model. We evaluate our method on artificial and real data.

==> extension.tex <==
\section{EXTENSION TO cDIVA}
\label{Extension}
\paragraph{Problem.} %The DVIB, as well as its copula extension described in Section~\ref{model} (cDVIB), enable us to calculate a non-linear compression $T$ of a random variable $X$ given a second random variable $Y$. However, the advantage of a non-linear generative IB comes with the serious limitation that the existing models are not fully generative. This means that the models can only generate the relevance variable $Y$ but not the input variable $X$. This property undermines the practicality of this model. For example, if a compression of an image $X$ given its label $Y$ were needed, the generative part would only allow us to sample new labels $Y$ given samples of the latent space $T$. 
The encoding and decoding neural networks defining $t$ implement highly non-linear transformations. It therefore becomes difficult to interpret the latent space as it is not clear in which areas of the latent space what properties of $x$ are preserved. A natural way to describe the latent space is to sample from it. However, in the plain DVIB model, one can only sample $y$, which does not provide any information about $x$. The cDIVA model solves this problem by allowing to sample not only $y$, but also $x$ from the latent representation. By examining the values of $x$ and $y$, sampled simultaneously for a given point in the latent space (e.g. a happy face has a happy emotion score), we can examine different areas of the latent space. In this manner we can assess both compression and relevance, both being crucial features of the Information Bottleneck method. This new property is essential for using the model in practice.

%Nevertheless, we would like to have a corresponding image to a label for two reasons. First, we cannot evaluate if the nonlinear compression $T$ samples reasonable labels because we do not have any information if the sampled label $Y$ corresponds to the image. This makes it difficult to evaluate if the compression $T$ generates meaningful samples of $Y$. Second, it is not possible to only employ the sampled relevance variable $Y$ without the input $X$ in many practical applications. 
%\begin{itemize}
%\item Advantage of DIB nonlinear compression also big disadvantage
%\item non linear leads to different latent spaces
%\item difficult to evaluate example labels and images dont know if compression works because one can only sample labels 
%\end{itemize}

\paragraph{Model extension.} In order to achieve the interpretability of the latent space motivated above, we propose a combined model with two decoder parts. The first decoder part is a cDVIB and the second decoder part is a VAE with a copula augmentation to guarantee the invariance property. Therefore, we refer to this model as \textit{copula Deep Information bottleneck Variational Autoencoder} (cDIVA). A sketch of the proposed model is illustrated in Figure \ref{fig:ib_vae}.
%Our model is closely related to the Deep Variational Canonical Correlation Analysis (DVCCA) model introduced by Wang \cite{WangLL16a}. Wang learns a latent representation $T$ given two views $X$ and $Y$ of the same image with two variational decoders.
Given both variables $x$ and $y$, we build a fully generative model that allows to evaluate the latent space $t$. It is therefore possible to see whether the latent space $t$ produces images $x$ and labels $y$ in a coherent manner.
%\begin{itemize}
%\item Proposed solution: Combination of the Deep Information Bottleneck and the Variational Autoencoder.
%\item Learn t given x and y
%\item One can sample x and y simultaneously and check if compression makes sense given an image
%\end{itemize}



cDIVA is again built upon the parametric IB formulation. In comparison to the previous model, we augment the parametric IB with a second mutual information term $I_{\phi,\tau}(t;x)$ that describes the VAE decoder part of our model. Therefore, the new parametric IB optimisation problem has the following form:

\begin{equation*}
\max_{\phi,\theta,\tau}  -I_{\phi}(t;\tilde{x}) + \lambda_1  I_{\phi,\theta}(t;\tilde{y}) + \lambda_2 I_{\phi,\tau}(t;\tilde{x}),
\end{equation*}
where the mutual informations stand for the encoder part (Eq.~(\ref{eq:ib:enc})) and the variational bounds for the decoders (Eq.~(\ref{eq:ib:dec}), Eq.~(\ref{eq:extDecItx})), respectively.


The added part is a VAE decoder. It is represented as the mutual information $I_{\phi,\tau}(t;x)$ which is derived by applying the same calculations as in Eq.~(\ref{eq:ib:dec}) with $x$ instead of $y$. We again use the mapping $\tilde{x_j} =\Phi^{-1}(\hat{F}(x_j))$ (see Eq.~(\ref{eq:transformation})) to guarantee the invariance property.


%\begin{equation}
%  \label{eq:extDecItx}
%  \begin{aligned}
%  I_{\phi,\tau}(T;X) &=\ D_{KL}\left(\left[\int p(t,x)\, \mathrm{d}x \right] \| p(t) p(x)\right)\\
%%  &=& \left[\int p_\phi(t|x) p(x)\, dx \right] \log \frac{p_\tau(x|t) p(t)}{ p(x) p(t)} \, \mathrm{d}y\,\mathrm{d}t\\
%&=\ \mathbb{E}_{p(x)} \int  p_\phi(t|x) \log p_\tau(x|t) \,\mathrm{d}t + h(Y)\\
%&=\ E_{p(x)} E_{p_\phi(t|x)}\log p_\tau(x|t)  + const,
%%&=\ i_{\phi,\tau}(T;X)  + \mbox{const.},
%\end{aligned}
%\end{equation}
\begin{equation}
  \label{eq:extDecItx}
  \begin{aligned}
  I_{\phi,\tau}(t;x) &=\ E_{p(x)} E_{p_\phi(t|x)}\log p_\tau(x|t)  + const,
\end{aligned}
\end{equation}

We use the reparametrisation tric~\citep{journals/corr/KingmaW13, Rezende} for both decoders to make inference feasible. We formulate the decoder part as a combination of two decoders, conditionally independent of each other given the latent space $t$. The cDVIB decoder has the form:
\begin{equation*}
\begin{aligned}
I(T;&Y) = \mathbb{E}_{p(x,y)} \mathbb{E}_{\epsilon \sim N(0,I)} \\
& \sum_j  \log  p_{\theta_j}(y_j|t = \mu_{k}(x) + diag(\sigma_k(x)) \epsilon) + \mbox{const.},
\end{aligned}
\end{equation*} 

and the VAE decoder:
\begin{equation*}
\begin{aligned}
I(T;&X) = \mathbb{E}_{p(x)} \mathbb{E}_{\epsilon \sim N(0,I)} \\ 
& \sum_j  \log  p_{\tau_j}(x_j|t = \mu_{k}(x) + diag(\sigma_k(x)) \epsilon) + \mbox{const.},
\end{aligned}
\end{equation*} 

The output distributions of both decoders are modelled as multivariate Gaussian distributions with diagonal covariance matrices. The parameters $\mu$ and $\Sigma$ are again implemented as DNNs.

%. We train this model on mini batches with stochastic gradient descent.



